UNICON: Combating Label Noise Through Uniform Selection and Contrastive Learning

Supervised deep learning methods require a large repository of annotated data; hence, label noise is inevitable. Training with such noisy data negatively impacts the generalization performance of deep neural networks. To combat label noise, recent state-of-the-art methods employ some sort of sample selection mechanism to select a possibly clean subset of data. Next, an off-the-shelf semi-supervised learning method is used for training where rejected samples are treated as unlabeled data. Our comprehensive analysis shows that current selection methods disproportionately select samples from easy (fast learnable) classes while rejecting those from relatively harder ones. This creates class imbalance in the selected clean set and in turn, deteriorates performance under high label noise. In this work, we propose UNICON, a simple yet effective sample selection method which is robust to high label noise. To address the disproportionate selection of easy and hard samples, we introduce a Jensen-Shannon divergence based uniform selection mechanism which does not require any probabilistic modeling and hyperparameter tuning. We complement our selection method with contrastive learning to further combat the memorization of noisy labels. Extensive experimentation on multiple benchmark datasets demonstrates the effectiveness of UNICON; we obtain an 11.4% improvement over the current state-of-the-art on CIFAR100 dataset with a 90% noise rate. Our code is publicly available

==> Alg1.tex <==
\begin{algorithm}[!t]
	
	\DontPrintSemicolon
	\small
	\textbf{Input:} Model-1 parameters $\theta^{(1)}$ and Model-2 parameters $\theta^{(2)}$, training set $(\mathcal{X},\mathcal{Y})$, number of samples $N$, number of classes $C$ \\
    
% 	$\theta^{(1)},\theta^{(2)}=\mathrm{WarmUp}(\mathcal{X},\mathcal{Y},\theta^{(1)},\theta^{(2)})$ \\
	
% 	\While{$t<\mathrm{num_epochs}$}  
% 	{
% 		\For{$k=1$ \KwTo  $2$}    
    % {  
	    \For{$i=1$ \KwTo  $N$}
	    {
    	    $\boldsymbol{\mathrm{p}}_i = \big(\mathrm{p_{model}}(\boldsymbol{x}_i;\theta^{(1)})+\mathrm{p_{model}}(\boldsymbol{x}_i;\theta^{(2)}\big)/2$ \\
    	    $\boldsymbol{d}_i = JSD(\boldsymbol{p}_i,\boldsymbol{y}_i)$ (see eq. \ref{eq:JSD}) \\
	    }
	   % $\mathcal{A}_{JSD} = \{d_b; b\in(1,...,N)\}$ 
	   \text{Determine R using eq.} \ref{eq:filter_rate} \\
	   $\mathcal{D}_{clean} = \{ \}$ \\
	   \For{$j=1$ \KwTo $C$}{
	    $\boldsymbol{d}^{(j)}_{sorted} = \text{Lower-Order-Sort}(\boldsymbol{d}^{(j)}) $ \\
	    $\boldsymbol{d}^{(j)}_{threshold} = \{d^{(j)}_l: l \in (1, \dots ,\frac{RN}{C})\} $\\
	    $\mathcal{D}^{(j)}_{clean} = \{ (\boldsymbol{x}^{(j)}_l,\boldsymbol{y}^{(j)}_l): \forall \hspace{0.1cm} d^{j}_l  \in \boldsymbol{d}^{j}_{threshold} \} $ \\
	    $\mathcal{D}_{clean} =  \mathcal{D}_{clean} \cup \mathcal{D}^{(j)}_{clean}$ \\
	    
	    }
	   % $\mathcal{W}    = Weight_Selection(\mathcal{A}_{JSD})$
	   % $\mathcal{W} = \{1 - \boldsymbol{d}_i; i \in (1, \dots , N) \}$ \\
	    $\mathcal{D}_{noisy} =  \mathcal{D} \setminus \mathcal{D}_{clean}$ \\
	    
	   % $\theta^{(k)} = SSL_{Training}(\mathcal{D}_{clean},\mathcal{D}_{noisy},\boldsymbol{d})$ \\
		
% 	}}
	\textbf{Output:} $\mathcal{D}_{noisy}, \mathcal{D}_{clean}$
	

	    
% 	$\mathcal{W} = \mathrm{JSD}(\mathcal{X},\mathcal{Y},\theta^{(1)},\theta^{(2)})$ \tcp*{Jensen-Shannon Distance between Ground Truths and Ensemble Outputs of $\theta^{(1)}$ $\theta^{(2)}$}
	
	
% 	$\bar{q}_{b}=\sum_{m}\big(\mathrm{p_{model}}(\hat{x};\theta^{(1)})+\mathrm{p_{model}}(\hat{u}^{weak}_{b,m};\theta^{(2)})\big)$
%     $ \mathcal{D}^{(clean)} = \mathrm{DBS}(\mathcal{W}, P)$ \tcp*{Distance Based Selection(DBS) of Clean Samples.}
    

%   \begin{algorithmic}
% 	   \IF{$e == E$}   
%     %\STATE
%           \STATE $\theta^{(1)},\theta^{(2)} = \mathrm{RCL}(\theta^{(1)},\theta^{(2)})$ \tcp*{after certain umber of epochs, re-initilize the classification layer}
%         \ENDIF
% 	\end{algorithmic}
	\caption{\small Uniform Selection}
	\label{alg:unicon}
	
\end{algorithm}

==> Alg2.tex <==
\begin{algorithm*}[!t]
	
	\DontPrintSemicolon
% 	\scriptsize
	\textbf{Input}: network-1 parameters $\theta^{(1)}$ and network-2 parameters $\theta^{(2)}$, training set $\mathbb{D} = (\mathcal{X},\mathcal{Y})$, number of samples $N$, number of classes $C$, %$\mathbb{D}_{clean}, \mathbb{D}_{noisy}, \boldsymbol{d}$, $\theta^{(1)}, \theta^{(2)}$,
	sharpening temperature $T$, unsupervised loss weight $\lambda_u$, contrastive loss weight $\lambda_c$  \\
	
	\For {$k=1$ \KwTo $2$}{
% 	$ \mathcal{X}^{(k)}_e = \{(x_i,y_i, w_i) | \forall (x_i,y_i), w_i \in \mathcal{D}^{(clean)}\}$ \\
% 	$\mathcal{U}^{(k)}_e = \{x_i , \forall (x_i) \in \mathcal{D}^{(noisy)}\}$ 
		\For {$\mathrm{iter}=1$ \KwTo $\mathrm{num\_iters}$}
		{
			From $\mathbb{D}^{(clean)}$, draw a mini-batch $\{(x_b,y_b);b\in(1,...,B)\}$ \\
			From $\mathbb{D}^{(noisy)}$, draw a mini-batch $\{u_b \leftarrow x_b ; b\in(1,...,B)\}$ \\
			\For{$b=1$ \KwTo $B$}
			{   
                \For{$m=1$ \KwTo $2$}
                {
                    $\hat{x}^{weak}_{b,m}=\mathrm{Weak-Augment}(x_b)$ \\ $\hat{u}^{weak}_{b,m}=\mathrm{Weak-Augment}(u_b)$  \\
        			$\hat{x}^{strong}_{b,m}=\mathrm{Strong-Augment}(x_b)$ \\
    				$\hat{u}^{strong}_{b,m}=\mathrm{Strong-Augment}(u_b)$  \\
                }
                
				${p}_{b}=\frac{1}{M}\sum_{m}\mathrm{p_{model}}(\hat{x}^{weak}_{b,m};\theta^{(k)})$  \\
				$\bar{y}_b=w_b y_b+(1-w_b){p}_{b}$ \tcp*{Label-refinement} \\
				 	
				$\hat{y}_b=\mathrm{Sharpen}(\bar{y}_b,T)$ 	\tcp*{ temperature sharpening}\\
				$\bar{q}_{b}=\frac{1}{2M}\sum_{m}\big(\mathrm{p_{model}}(\hat{u}^{weak}_{b,m};\theta^{(1)})+\mathrm{p_{model}}(\hat{u}^{weak}_{b,m};\theta^{(2)})\big)$
				 \tcp*{Pseudo-label} \\
				${q}_{b}=\mathrm{Sharpen}(\bar{q}_{b},T)$ \tcp*{temperature sharpening} \\
			}
			$\hat{\mathbb{X}}=\{(\hat{x}^{strong}_{b,m},\hat{y}_b);b\in(1,...,B)\}$ \\
			$\hat{\mathbb{U}}=\{(\hat{u}^{strong}_{b,m},q_{b});b\in(1,...,B)\}$ \\
	        $\mathcal{L}_\mathcal{X},\mathcal{L}_\mathcal{U}=\mathrm{MixMatch}(\hat{\mathcal{X}},\hat{\mathcal{U}})$ \tcp*{apply MixMatch}
	        $\mathcal{L}_\mathcal{C} = \mathcal{L}_{con}\big(\hat{u}^{strong}_{b,1},\hat{u}^{strong}_{b,2} ;b\in(1,...,B)\big)$ \\
			$\mathcal{L}=\mathcal{L}_\mathcal{X}+ \lambda_u \mathcal{L}_\mathcal{U}+ \lambda_c \mathcal{L}_\mathcal{C}+ \lambda_r \mathcal{L}_\mathrm{reg}$ \tcp*{total loss} \\
			$\theta^{(k)}=\mathrm{SGD}(\mathcal{L},\theta^{(k)})$ 
			}
		}
	    \textbf{Return:} Updated $\theta^{(k)}$
	\caption{\small SSL Training}
	\label{alg:SSL_training}
	
\end{algorithm*}


% \begin{algorithm}[!t]
	
% 	\DontPrintSemicolon
% 	\scriptsize
% 	$ \mathcal{X}^{(k)}_e = \{(x_i,y_i) | \forall (x_i,y_i) \in \mathcal{D}^{(clean)}\}$\tcp*{labeled training set for $\theta^{(k)}$}
% 	$\mathcal{U}^{(k)}_e = \{x_i , \forall (x_i) \not \in \mathcal{D}^{(clean)}\}$  \tcp*{unlabeled training set for $\theta^{(k)}$}
    	
% 		\For {$\mathrm{iter}=1$ \KwTo $\mathrm{num\_iters}$}
% 		{
% 			From $\mathcal{X}^{(k)}_e$, draw a mini-batch $\{(x_b,y_b);b\in(1,...,B)\}$ \\
% 			From $\mathcal{U}^{(k)}_e$, draw a mini-batch $\{u_b;b\in(1,...,B)\}$ \\
% 			\For{$b=1$ \KwTo $B$}
% 			{   

% 				$\hat{x}^{strong}_{b,m}=\mathrm{StrongAugment}(x_b)$  \tcp*{apply strong augmentation to $x_b$}

% 				$\hat{u}^{strong}_{b,m}=\mathrm{StrongAugment}(u_b)$  \tcp*{apply strong augmentation to $u_b$}
%                 \For{$m=1$ \KwTo $2$}
%                 {
%     				$\hat{x}^{weak}_{b,m}=\mathrm{WeakAugment}(x_b)$  \tcp*{apply $m^{th}$ round of weak augmentation to $x_b$}				
%     				$\hat{u}^{weak}_{b,m}=\mathrm{WeakAugment}(u_b)$  \tcp*{apply $m^{th}$ round of weak augmentation to $u_b$}
%                 }
                
% 				${p}_{b}=\frac{1}{M}\sum_{m}\mathrm{p_{model}}(\hat{x}^{weak}_{b,m};\theta^{(k)})$ \tcp*{average the predictions across augmentations of $x_b$}
% 				$\bar{y}_b=\Gamma y_b+(1-\Gamma){p}_{b}$ \\
% 				 	\tcp*{refine ground-truth label guided by the refinement coefficient}
% 				$\hat{y}_b=\mathrm{Sharpen}(\bar{y}_b,T)$ 	\tcp*{apply temperature sharpening to the refined label}
% 				$\bar{q}_{b}=\frac{1}{2M}\sum_{m}\big(\mathrm{p_{model}}(\hat{u}^{weak}_{b,m};\theta^{(1)})+\mathrm{p_{model}}(\hat{u}^{weak}_{b,m};\theta^{(2)})\big)$\\
% 				 \tcp*{co-guessing: average the predictions from both networks across weak augmentations of $u_b$}
% 				%$\bar{q}_{b}=\frac{1}{M}\sum_{m}\mathrm{p_{model}}(\hat{u}_{b,m};\theta^{(z)})$ \tcp*{average the predictions across augmentations of $u_b$}
% 				${q}_{b}=\mathrm{Sharpen}(\bar{q}_{b},T)$		\tcp*{apply temperature sharpening to the guessed label}		    
% 			}
% 			$\hat{\mathcal{X}}=\{(\hat{x}^{strong}_{b},\hat{y}_b);b\in(1,...,B)\}$	\tcp*{strongly augmented labeled mini-batch}
% 			$\hat{\mathcal{U}}=\{(\hat{u}^{strong}_{b,m},q_{b});b\in(1,...,B)\}$	\tcp*{strongly augmented unlabeled mini-batch}
% 	        $\mathcal{L}_\mathcal{X},\mathcal{L}_\mathcal{U}=\mathrm{MixMatch}(\hat{\mathcal{X}},\hat{\mathcal{U}})$ \tcp*{apply MixMatch}
% 			$\mathcal{L}=\mathcal{L}_\mathcal{X}+\lambda_u \mathcal{L}_\mathcal{U}+\lambda_r \mathcal{L}_\mathrm{reg}$ \tcp*{total loss}
% 			$\theta^{(k)}=\mathrm{SGD}(\mathcal{L},\theta^{(k)})$  \tcp*{update model parameters}}
% 	\caption{\small Robust Noisy Label Learning}
% 	\label{alg:dividemix}
	
% \end{algorithm}
